Achieving Reliable Human Assessment of Open-Domain Dialogue Systems

Evaluation of open-domain dialogue systems is highly challenging and development of better techniques is highlighted time and again as desperately needed. Despite substantial efforts to carry out reliable live evaluation of systems in recent competitions, annotations have been abandoned and reported as too unreliable to yield sensible results. This is a serious problem since automatic metrics are not known to provide a good indication of what may or may not be a high-quality conversation. Answering the distress call of competitions that have emphasized the urgent need for better evaluation techniques in dialogue, we present the successful development of human evaluation that is highly reliable while still remaining feasible and low cost. Self-replication experiments reveal almost perfectly repeatable results with a correlation of $r=0.969$. Furthermore, due to the lack of appropriate methods of statistical significance testing, the likelihood of potential improvements to systems occurring due to chance is rarely taken into account in dialogue evaluation, and the evaluation we propose facilitates application of standard tests. Since we have developed a highly reliable evaluation method, new insights into system performance can be revealed. We therefore include a comparison of state-of-the-art models (i) with and without personas, to measure the contribution of personas to conversation quality, as well as (ii) prescribed versus freely chosen topics. Interestingly with respect to personas, results indicate that personas do not positively contribute to conversation quality as expected.

==> fig-01-indiv-agree-r.tex <==
% \begin{tabular}{cc}
% \multirow{3}{*}{\rotatebox[origin=b]{90}{\parbox[c]{6cm}{\centering \small \# workers \hspace{2cm}}}} \\
% % & \includegraphics[width=0.3\textwidth]{fig/rater-agreement/corr_z_qc.png}  \\
% & \includegraphics[width=0.3\textwidth]{fig/rater-agreement/corr_z_qc.pdf}  \\
%      & \small $r$ \\
% \end{tabular}

\includegraphics[width=0.495\textwidth]{fig/rater-agreement/corr_z_qc.pdf}

==> old-sec-00-abstract.tex <==
\begin{abstract}
  Evaluation is a known open problem in open domain dialogue and has been highlighted as  negatively impacting system development. In contrast to other tasks, for which hand-crafted references are straight-forward to produce, there exists no such reference for dialogue systems, but instead an extremely large number of possible correct responses for each input from the user. This vast number of  possible correct responses causes substantial challenges for evaluation, as well as difficulties with respect to taking dialogue history into account. Human evaluation is unfortunately not guaranteed to overcome challenges as human assessors of systems can lack reliability. In this paper, we propose a new method of evaluation of dialogue systems that (i) avoids the need for pre-created references and takes dialogue history into account; (ii) overcomes challenges with respect to reliability; (iii) is highly cost effect; (iv) can be carried out on a very large scale. Our proposed human evaluation employs a continuous rating scale to allow score distributions to be collected from crowd-sourced human assessors. We develop a quality control mechanism that allows human assessors with low consistency to be filtered out, comparing only the judgement of each assessor with his/her own previous judgements. Self-replication experiments reveal our proposed method to be highly reliable, correlating almost perfectly at $r=0.969$ in repeat evaluations.\footnote{The protocol employed in this work was approved by the ANONYMOUS Research Ethics Committee.}
  %under the category of notification only and was given a waiver of the requirement for signed consent because it is an anonymous online survey.}
    
\end{abstract}

==> orig-dens-plots.tex <==
\begin{figure*}
    \centering


    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/rater-agreement/corr_z_qc.png}
        \caption{DA}
        \label{fig:boxplot-ft-z-overall}
    \end{subfigure}\hspace{0em}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/rater-agreement/corr_l2_qc.png}
        \caption{2-point}
    \end{subfigure}\hspace{0em}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/rater-agreement/corr_l4_qc.png}
        \caption{4-point}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/rater-agreement/corr_l5_qc.png}
        \caption{5-point}
        \label{fig:boxplot-ft-z-overall}
    \end{subfigure}\hspace{0em}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/rater-agreement/corr_l10_qc.png}
        \caption{10-point}
    \end{subfigure}\hspace{0em}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \raisebox{5em}{
            \includegraphics[width=0.5\textwidth]{fig/rater-agreement/legend.png}
        }
        % \includegraphics[width=\textwidth]{fig/rater-agreement/legend.png}
        
    \end{subfigure}
    
    \caption{The histogram with kernel density estimate (KDE) plot describing the distribution of correlations on DA scores and $n$-point Likert scores for both passed and failed workers}
    \label{fig:correlation-distribution}
\end{figure*}

==> sec-09-qc-fail-details.tex <==
\subsection{Quality control that fails}
At first, we decide to insert a task of image recognition within each conversation as our quality control method. 
In detail, we firstly extract images whose caption belongs to a set of certain topics from the Image Caption Quality Dataset\footnote{https://github.com/google-research-datasets/Image-Caption-Quality-Dataset}, then these images are stored as our quality-control dataset. 
We hope the captions of images should clear enough, so the list of certain topics in our experiment is: Rainbow, Football, Flower, Candy, Coffee, House, Snow, Dog and Cat. Figure \ref{fig:qc-old} shows an example of failed quality control, the quality-control image for is a cup of coffee so the worker is expected to answer "Coffee". First the system will show the image and ask the worker to answer what the image is about during the conversation as shown in Figure \ref{fig:qc-old1}, and the worker should send the answer to the system. After that, the system will record the answer, and continue the conversation by repeating the utterance before the quality control(see Figure \ref{fig:qc-old2}).

However, our preliminary research shows this method does not work very well since we found the pass rate of this mechanism is almost 100\%. This is probably because the intention is too obvious that a worker can easily pass it. Hence we decided to give up this method, and turn to a stricter statistic-based quality control method.

==> tables/tbl-02-FreeAndGiven.tex <==

\begin{tabular}{clcccccccccccc}
\toprule
%\multicolumn{10}{c}{Free Topic} \bigstrut\\

&\rotatebox{60}{Model} & $n$ & \rotatebox{60}{Overall} && \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic $\downarrow$} & \rotatebox{60}{Repetitive $\downarrow$} \bigstrut\\
\midrule
\multirow{10}*{\rotatebox{90}{Free Topic}}

&A          & 798  & 52.49 && 53.03  & 54.07  & 58.12  & 61.78  & 65.24  & 35.73  & 39.47 \\
&B          & 798  & 50.41 && 51.39  & 51.68  & 56.37  & 64.50  & 67.84  & 25.63  & 35.45 \\
&A$_p$          & 707  & 45.53 && 47.38  & 46.23  & 48.52  & 60.17  & 47.50  & 28.30  & 40.62 \\
&C          & 791  & 43.96 && 50.50  & 47.53  & 35.85  & 55.73  & 33.98  & 27.35  & 56.76 \\
&C$_p$          & 714  & 41.21 && 47.13  & 46.26  & 39.25  & 55.05  & 32.07  & 21.85  & 46.84 \\
&B$_p$          & 707  & 39.93 && 41.35  & 40.06  & 44.93  & 53.74  & 43.72  & 25.25  & 30.49 \\
&D          & 707  & 33.71 && 30.28  & 29.95  & 41.72  & 45.92  & 49.07  & 17.30  & 21.72 \\
&D$_p$          & 798  & 29.38 && 26.19  & 27.97  & 37.53  & 44.19  & 35.26  & 17.46  & 17.06 \\
&E$_p$          & 763  & 28.65 && 29.34  & 28.50  & 29.13  & 47.07  & 21.30  & 17.82  & 27.41 \\
&E          & 742  & 28.99 && 30.75  & 30.65  & 31.27  & 46.42  & 23.60  & 15.10  & 25.13 \\
\midrule

%\multicolumn{10}{c}{Known Topic} \bigstrut\\


%\midrule
\multirow{10}*{\rotatebox{90}{Known Topic}} 
&A          & 721  & 53.43 && 53.65  & 52.35  & 63.24  & 67.28  & 66.97  & 28.17  & 42.32 \\
&B          & 742  & 49.55 && 49.23  & 47.76  & 57.79  & 60.64  & 62.22  & 32.56  & 36.65 \\
&A$_p$          & 721  & 50.21 && 54.53  & 53.50  & 52.84  & 58.83  & 53.18  & 38.87  & 39.70 \\
&C          & 784  & 47.93 && 56.18  & 53.69  & 43.15  & 56.88  & 40.46  & 29.61  & 55.54 \\
&C$_p$          & 658  & 42.41 && 47.98  & 45.48  & 37.66  & 54.51  & 32.50  & 26.00  & 52.72 \\
&B$_p$          & 700  & 44.94 && 48.83  & 46.70  & 49.58  & 55.86  & 49.21  & 25.82  & 38.61 \\
&D          & 728  & 35.14 && 30.32  & 33.13  & 42.90  & 49.92  & 48.51  & 20.11  & 21.09 \\
&D$_p$          & 714  & 27.22 && 22.56  & 22.53  & 35.22  & 41.70  & 34.98  & 17.44  & 16.09 \\
&E$_p$          & 721  & 31.58 && 31.73  & 30.82  & 35.44  & 47.12  & 27.06  & 21.90  & 26.97 \\
&E          & 721  & 30.09 && 33.17  & 31.95  & 31.14  & 47.12  & 24.90  & 19.10  & 23.23 \\

\midrule

%      &       &       &       &       &       &       &       &       &  \bigstrut\\
%\hline
%\multicolumn{10}{c}{Correlation between Rounds 1 and 2} \bigstrut\\
%\midrule
\multicolumn{2}{c}{$r$} & $-$ & 0.970  && 0.955  & 0.918  & 0.949  & 0.928  & 0.972  & 0.738  & 0.968  \bigstrut[t]\\
%\multicolumn{2}{c}{Spearman} & $-$ & 0.927  && 0.879  & 0.830  & 0.879  & 0.945  & 0.927  & 0.867  & 0.976  \bigstrut[b]\\
\bottomrule
\end{tabular}%


==> tables/tbl-02-corr-FreeAndGiven.tex <==

\begin{tabular}{clcccccccccccc}
\toprule
%\multicolumn{10}{c}{Free Topic} \bigstrut\\

&\rotatebox{60}{Model} & $n$ & \rotatebox{60}{Overall} && \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic $\downarrow$} & \rotatebox{60}{Repetitive $\downarrow$} \bigstrut\\
\midrule
\multirow{10}*{\rotatebox{90}{Free Topic}}

&A          & 798  & 52.49 && 53.03  & 54.07  & 58.12  & 61.78  & 65.24  & 35.73  & 39.47 \\
&B          & 798  & 50.41 && 51.39  & 51.68  & 56.37  & 64.50  & 67.84  & 25.63  & 35.45 \\
&A$_p$          & 707  & 45.53 && 47.38  & 46.23  & 48.52  & 60.17  & 47.50  & 28.30  & 40.62 \\
&C          & 791  & 43.96 && 50.50  & 47.53  & 35.85  & 55.73  & 33.98  & 27.35  & 56.76 \\
&C$_p$          & 714  & 41.21 && 47.13  & 46.26  & 39.25  & 55.05  & 32.07  & 21.85  & 46.84 \\
&B$_p$          & 707  & 39.93 && 41.35  & 40.06  & 44.93  & 53.74  & 43.72  & 25.25  & 30.49 \\
&D          & 707  & 33.71 && 30.28  & 29.95  & 41.72  & 45.92  & 49.07  & 17.30  & 21.72 \\
&D$_p$          & 798  & 29.38 && 26.19  & 27.97  & 37.53  & 44.19  & 35.26  & 17.46  & 17.06 \\
&E$_p$          & 763  & 28.65 && 29.34  & 28.50  & 29.13  & 47.07  & 21.30  & 17.82  & 27.41 \\
&E          & 742  & 28.99 && 30.75  & 30.65  & 31.27  & 46.42  & 23.60  & 15.10  & 25.13 \\
\midrule

%\multicolumn{10}{c}{Known Topic} \bigstrut\\


%\midrule
\multirow{10}*{\rotatebox{90}{Known Topic}} 
&A          & 721  & 53.43 && 53.65  & 52.35  & 63.24  & 67.28  & 66.97  & 28.17  & 42.32 \\
&B          & 742  & 49.55 && 49.23  & 47.76  & 57.79  & 60.64  & 62.22  & 32.56  & 36.65 \\
&A$_p$          & 721  & 50.21 && 54.53  & 53.50  & 52.84  & 58.83  & 53.18  & 38.87  & 39.70 \\
&C          & 784  & 47.93 && 56.18  & 53.69  & 43.15  & 56.88  & 40.46  & 29.61  & 55.54 \\
&C$_p$          & 658  & 42.41 && 47.98  & 45.48  & 37.66  & 54.51  & 32.50  & 26.00  & 52.72 \\
&B$_p$          & 700  & 44.94 && 48.83  & 46.70  & 49.58  & 55.86  & 49.21  & 25.82  & 38.61 \\
&D          & 728  & 35.14 && 30.32  & 33.13  & 42.90  & 49.92  & 48.51  & 20.11  & 21.09 \\
&D$_p$          & 714  & 27.22 && 22.56  & 22.53  & 35.22  & 41.70  & 34.98  & 17.44  & 16.09 \\
&E$_p$          & 721  & 31.58 && 31.73  & 30.82  & 35.44  & 47.12  & 27.06  & 21.90  & 26.97 \\
&E          & 721  & 30.09 && 33.17  & 31.95  & 31.14  & 47.12  & 24.90  & 19.10  & 23.23 \\

\midrule

%      &       &       &       &       &       &       &       &       &  \bigstrut\\
%\hline
%\multicolumn{10}{c}{Correlation between Rounds 1 and 2} \bigstrut\\
%\midrule
\multicolumn{2}{c}{$r$} & $-$ & 0.970  && 0.955  & 0.918  & 0.949  & 0.928  & 0.972  & 0.738  & 0.968  \bigstrut[t]\\
%\multicolumn{2}{c}{Spearman} & $-$ & 0.927  && 0.879  & 0.830  & 0.879  & 0.945  & 0.927  & 0.867  & 0.976  \bigstrut[b]\\
\bottomrule
\end{tabular}%


==> tables/tbl-02-corr-FreeAndGiven_bkp2.tex <==

\begin{tabular}{cccccccccc}
\hline
\multicolumn{10}{c}{Free Topic} \bigstrut\\
\hline
\textbf{Model} & \textbf{N} & \textbf{Overall} & \textbf{Interesting} & \textbf{Fun} & \textbf{Consistent} & \textbf{Fluent} & \textbf{Topic} & \textbf{Robotic $\downarrow$} & \textbf{Repetitive$\downarrow$} \bigstrut\\
\hline
A$_n$    & 287   & 55.90 & 63.39  & 64.46  & 61.41  & 70.46  & 68.56  & 71.02  & 65.95  \bigstrut[t]\\
B$_n$    & 315   & 53.82 & 57.67  & 59.96  & 57.60  & 68.38  & 66.64  & 66.76  & 66.78  \\
A$_p$    & 315   & 52.46 & 61.60  & 61.44  & 53.67  & 62.87  & 54.51  & 68.98  & 57.87  \\
B$_p$    & 259   & 52.41 & 60.30  & 59.84  & 59.16  & 64.76  & 60.62  & 69.57  & 68.24  \\
C$_p$   & 273   & 48.52 & 55.72  & 55.26  & 45.64  & 62.56  & 36.95  & 70.92  & 45.56  \\
C$_n$    & 322   & 48.26 & 57.15  & 56.80  & 48.98  & 56.74  & 47.09  & 73.46  & 55.48  \\
D$_n$    & 308   & 43.38 & 45.98  & 44.64  & 52.43  & 53.32  & 59.02  & 78.82  & 72.93  \\
D$_p$    & 280   & 36.59 & 37.33  & 38.38  & 43.38  & 51.67  & 37.23  & 71.55  & 80.32  \\
E$_p$    & 245   & 35.74 & 39.40  & 38.31  & 41.43  & 54.63  & 28.77  & 77.94  & 74.43  \\
E$_n$    & 371   & 34.68 & 37.40  & 39.21  & 40.28  & 54.02  & 31.23  & 79.02  & 80.38  \bigstrut[b]\\
\hline
      &       &       &       &       &       &       &       &       &  \bigstrut\\
\hline
\multicolumn{10}{c}{Given topic} \bigstrut\\
\hline
\textbf{Model} & \textbf{N} & \textbf{Overall} & \textbf{Interesting} & \textbf{Enjoyable} & \textbf{Consistency} & \textbf{Fluency} & \textbf{Stick} & \textbf{Obviousness$\downarrow$} & \textbf{Repetitive$\downarrow$} \bigstrut\\
\hline
A$_n$    & 308   & 54.11 & 56.32  & 53.20  & 59.41  & 65.18  & 64.39  & 69.61  & 50.11  \bigstrut[t]\\
B$_n$    & 336   & 48.09 & 49.06  & 47.17  & 55.73  & 57.04  & 61.08  & 69.71  & 63.73  \\
A$_p$    & 315   & 51.36 & 54.60  & 53.67  & 54.93  & 62.71  & 51.60  & 64.69  & 53.33  \\
B$_p$    & 287   & 45.51 & 49.95  & 47.20  & 49.37  & 57.51  & 46.88  & 71.37  & 60.95  \\
C$_p$    & 287   & 37.62 & 40.95  & 38.78  & 33.76  & 47.34  & 29.66  & 76.63  & 50.49  \\
C$_n$    & 336   & 49.92 & 59.67  & 56.23  & 47.50  & 55.46  & 43.90  & 69.67  & 43.65  \\
D$_n$    & 315   & 36.83 & 33.62  & 34.40  & 43.31  & 51.11  & 44.51  & 75.22  & 73.89  \\
D$_p$    & 308   & 25.37 & 18.57  & 20.84  & 34.91  & 37.39  & 31.09  & 83.32  & 81.91  \\
E$_p$    & 273   & 32.68 & 31.10  & 31.23  & 35.92  & 43.72  & 27.77  & 76.97  & 63.97  \\
E$_n$    & 350   & 30.44 & 34.12  & 32.34  & 32.30  & 44.46  & 26.96  & 81.42  & 75.66  \bigstrut[b]\\
\hline
      &       &       &       &       &       &       &       &       &  \bigstrut\\
\hline
\multicolumn{10}{c}{Correlation between above two} \bigstrut\\
\hline
\multicolumn{2}{c}{$r$} & 0.9142  & 0.9022  & 0.9042  & 0.9150  & 0.7988  & 0.9531  & 0.5521  & 0.8559  \bigstrut[t]\\
%\multicolumn{2}{c}{Spearman} & 0.8667  & 0.8424  & 0.8424  & 0.9030  & 0.8424  & 0.9515  & 0.5515  & 0.9030  \bigstrut[b]\\
\hline
\end{tabular}%


==> tables/tbl-02b-free-known-z.tex <==

\begin{tabular}{clcccccccccccc}
\toprule
%\multicolumn{10}{c}{Free Topic} \bigstrut\\

%&\rotatebox{60}{Model} & $z$ && \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic $\downarrow$} & \rotatebox{60}{Repetitive $\downarrow$} \bigstrut\\
& Model & Overall && Interesting & Fun & Consistent & Fluent & Topic & Robotic$\downarrow$ & Repetitive$\downarrow$ \\

%\midrule
%\multirow{10}*{\rotatebox{90}{Free Topic}} \\
%&A            & 0.534 && 0.564  & 0.602  & 0.711  & 0.863  & 0.964  & -0.038  & 0.069 \\
%&B            & 0.419 && 0.474  & 0.481  & 0.614  & 0.875  & 0.994  & -0.431  & -0.075 \\
%&A$_p$            & 0.318 && 0.399  & 0.372  & 0.443  & 0.821  & 0.404  & -0.330  & 0.116 \\
%&C            & 0.262 && 0.491  & 0.379  & 0.028  & 0.636  & -0.066  & -0.316  & 0.680 \\
%&C$_p$            & 0.189 && 0.409  & 0.373  & 0.159  & 0.672  & -0.114  & -0.521  & 0.349 \\
%&B$_p$            & 0.173 && 0.230  & 0.197  & 0.369  & 0.673  & 0.320  & -0.395  & -0.187 \\
%&D            & -0.087 && -0.190  & -0.208  & 0.166  & 0.311  & 0.401  & -0.637  & -0.449 \\
%&D$_p$            & -0.201 && -0.308  & -0.234  & 0.092  & 0.312  & 0.025  & -0.625  & -0.669 \\
%&E$_p$            & -0.217 && -0.181  & -0.201  & -0.196  & 0.380  & -0.455  & -0.605  & -0.264 \\
%&E            & -0.243 && -0.165  & -0.160  & -0.142  & 0.329  & -0.407  & -0.745  & -0.411 \\

\midrule

%\multicolumn{10}{c}{Known Topic} \bigstrut\\


%\midrule
\multirow{10}*{\rotatebox{90}{Known Topic}} \\
&A            & 0.552 && 0.565  & 0.527  & 0.873  & 1.018  & 1.011  & -0.287  & 0.156 \\
&B            & 0.376 && 0.379  & 0.340  & 0.634  & 0.769  & 0.820  & -0.221  & -0.087 \\
&A$_p$            & 0.422 && 0.589  & 0.560  & 0.518  & 0.718  & 0.527  & 0.009  & 0.034 \\
&C            & 0.322 && 0.615  & 0.537  & 0.190  & 0.631  & 0.061  & -0.344  & 0.565 \\
&C$_p$            & 0.222 && 0.402  & 0.337  & 0.089  & 0.654  & -0.068  & -0.376  & 0.514 \\
&B$_p$            & 0.273 && 0.406  & 0.340  & 0.414  & 0.633  & 0.423  & -0.369  & 0.063 \\
&D            & -0.139 && -0.277  & -0.204  & 0.123  & 0.349  & 0.295  & -0.638  & -0.620 \\
&D$_p$            & -0.267 && -0.426  & -0.402  & -0.011  & 0.234  & 0.000  & -0.628  & -0.636 \\
&E$_p$            & -0.198 && -0.172  & -0.203  & -0.054  & 0.316  & -0.343  & -0.533  & -0.396 \\
&E            & -0.240 && -0.125  & -0.161  & -0.196  & 0.318  & -0.393  & -0.631  & -0.489 \\


\midrule

%      &       &       &       &       &       &       &       &       &  \bigstrut\\
%\hline
%\multicolumn{10}{c}{Correlation between Rounds 1 and 2} \bigstrut\\
%\midrule
\multicolumn{2}{c}{$r$ } &0.984  && 0.967  & 0.944  & 0.958  & 0.951  & 0.981  & 0.715  & 0.950 \bigstrut[t]\\
%\multicolumn{2}{c}{Spearman} & 0.939  && 0.830  & 0.770  & 0.915  & 0.891  & 0.952  & 0.855  & 0.939 \bigstrut[b]\\
\bottomrule
\end{tabular}%


==> tables/tbl-02c-free-free-raw.tex <==

\begin{tabular}{clcccccccccccc}
\toprule
%\multicolumn{10}{c}{Free Topic} \bigstrut\\

&\rotatebox{60}{Model} & $n$ & \rotatebox{60}{Overall} && \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic $\downarrow$} & \rotatebox{60}{Repetitive $\downarrow$} \bigstrut\\
\midrule
\multirow{10}*{\rotatebox{90}{Run 1 - Free Topic}}

&A          & 798  & 52.49 && 53.03  & 54.07  & 58.12  & 61.78  & 65.24  & 35.73  & 39.47 \\
&B          & 798  & 50.41 && 51.39  & 51.68  & 56.37  & 64.50  & 67.84  & 25.63  & 35.45 \\
&A$_p$          & 707  & 45.53 && 47.38  & 46.23  & 48.52  & 60.17  & 47.50  & 28.30  & 40.62 \\
&C          & 791  & 43.96 && 50.50  & 47.53  & 35.85  & 55.73  & 33.98  & 27.35  & 56.76 \\
&C$_p$          & 714  & 41.21 && 47.13  & 46.26  & 39.25  & 55.05  & 32.07  & 21.85  & 46.84 \\
&B$_p$          & 707  & 39.93 && 41.35  & 40.06  & 44.93  & 53.74  & 43.72  & 25.25  & 30.49 \\
&D          & 707  & 33.71 && 30.28  & 29.95  & 41.72  & 45.92  & 49.07  & 17.30  & 21.72 \\
&D$_p$          & 798  & 29.38 && 26.19  & 27.97  & 37.53  & 44.19  & 35.26  & 17.46  & 17.06 \\
&E$_p$          & 763  & 28.65 && 29.34  & 28.50  & 29.13  & 47.07  & 21.30  & 17.82  & 27.41 \\
&E          & 742  & 28.99 && 30.75  & 30.65  & 31.27  & 46.42  & 23.60  & 15.10  & 25.13 \\
\midrule

%\multicolumn{10}{c}{Known Topic} \bigstrut\\


%\midrule
\multirow{10}*{\rotatebox{90}{Run 2 - Free Topic}} 

&A          & 623  & 51.67 && 56.62  & 56.27  & 59.21  & 64.69  & 64.04  & 27.11  & 33.74 \\
&B          & 539  & 49.07 && 52.42  & 50.66  & 54.88  & 60.86  & 63.73  & 29.57  & 31.38 \\
&A$_p$          & 553  & 50.56 && 59.95  & 60.23  & 54.28  & 60.61  & 52.06  & 27.59  & 39.22 \\
&C          & 630  & 45.87 && 55.60  & 53.02  & 45.16  & 54.70  & 38.72  & 24.40  & 49.50 \\
&C$_p$          & 539  & 42.27 && 51.19  & 49.61  & 37.90  & 54.17  & 30.42  & 22.74  & 49.84 \\
&B$_p$          & 609  & 46.71 && 51.92  & 49.95  & 54.62  & 56.01  & 52.85  & 28.48  & 33.10 \\
&D          & 595  & 38.17 && 38.31  & 35.39  & 50.99  & 46.38  & 57.94  & 16.09  & 22.08 \\
&D$_p$          & 567  & 30.89 && 31.07  & 30.37  & 38.37  & 44.64  & 31.47  & 21.85  & 18.48 \\
&E$_p$          & 511  & 31.66 && 33.63  & 33.26  & 38.77  & 51.53  & 26.99  & 17.63  & 19.79 \\
&E          & 679  & 31.70 && 35.67  & 36.32  & 35.26  & 46.91  & 26.79  & 18.98  & 21.99 \\
%\midrule

%      &       &       &       &       &       &       &       &       &  \bigstrut\\
\hline


\multicolumn{2}{c}{$r$} & $-$ &  0.959  && 0.947  & 0.919  & 0.880  & 0.951  & 0.951  & 0.783  & 0.945 \bigstrut[t]\\
%\multicolumn{2}{c}{Spearman} & $-$ & 0.915  && 0.891  & 0.842  & 0.842  & 0.952  & 0.952  & 0.745  & 0.927  \bigstrut[b]\\
\bottomrule
\end{tabular}%


==> tables/tbl-02d-free-free-z.tex <==

\begin{tabular}{clrrrrrrrrrrrrrrrrrrrrrrrrrrcccccccccccc}
\toprule
%\multicolumn{10}{c}{Free Topic} \bigstrut\\

%&\rotatebox{20}{Model} & {$z$} && \rotatebox{20}{Interesting} & \rotatebox{20}{Fun} & \rotatebox{20}{Consistent} & \rotatebox{20}{Fluent} & \rotatebox{20}{Topic} & \rotatebox{20}{Robotic $\downarrow$} & \rotatebox{20}{Repetitive $\downarrow$} \bigstrut\\

% & Model & Overall && Interesting & Fun & Consistent & Fluent & Topic & Robotic$\downarrow$ & Repetitive$\downarrow$ \\
&\rotatebox{60}{Model} & \rotatebox{60}{Overall} && \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic $\downarrow$} & \rotatebox{60}{Repetitive $\downarrow$} \bigstrut\\
\midrule
\multirow{10}*{\rotatebox{90}{Run 1 - Free Topic}}

&A            & 0.534 && 0.564  & 0.602  & 0.711  & 0.863  & 0.964  & $-$0.038  & 0.069 \\
&B            & 0.419 && 0.474  & 0.481  & 0.614  & 0.875  & 0.994  & $-$0.431  & $-$0.075 \\
&A$_p$        & 0.318 && 0.399  & 0.372  & 0.443  & 0.821  & 0.404  & $-$0.330  & 0.116 \\
&C            & 0.262 && 0.491  & 0.379  & 0.028  & 0.636  & $-$0.066  & $-$0.316  & 0.680 \\
&C$_p$        & 0.189 && 0.409  & 0.373  & 0.159  & 0.672  & $-$0.114  & $-$0.521  & 0.349 \\
&B$_p$        & 0.173 && 0.230  & 0.197  & 0.369  & 0.673  & 0.320  & $-$0.395  & $-$0.187 \\
&D            & $-$0.087 && $-$0.190  & $-$0.208  & 0.166  & 0.311  & 0.401  & $-$0.637  & $-$0.449 \\
&D$_p$        & $-$0.201 && $-$0.308  & $-$0.234  & 0.092  & 0.312  & 0.025  & $-$0.625  & $-$0.669 \\
&E$_p$        & $-$0.217 && $-$0.181  & $-$0.201  & $-$0.196  & 0.380  & $-$0.455  & $-$0.605  & $-$0.264 \\
&E            & $-$0.243 && $-$0.165  & $-$0.160  & $-$0.142  & 0.329  & $-$0.407  & $-$0.745  & $-$0.411 \\
%\midrule

%\multicolumn{10}{c}{Known Topic} \bigstrut\\


\midrule
\multirow{10}*{\rotatebox{90}{Run 2 - Free Topic}} 
&A            & 0.455 && 0.635  & 0.629  & 0.728  & 0.924  & 0.922  & $-$0.443  & $-$0.212 \\
&B            & 0.344 && 0.464  & 0.407  & 0.554  & 0.763  & 0.822  & $-$0.338  & $-$0.266 \\
&A$_p$        & 0.423 && 0.747  & 0.763  & 0.555  & 0.728  & 0.474  & $-$0.348  & 0.040 \\
&C            & 0.245 && 0.576  & 0.492  & 0.229  & 0.585  & 0.043  & $-$0.545  & 0.337 \\
&C$_p$        & 0.154 && 0.453  & 0.390  & 0.027  & 0.544  & $-$0.200  & $-$0.515  & 0.382 \\
&B$_p$        & 0.260 && 0.464  & 0.372  & 0.560  & 0.581  & 0.496  & $-$0.412  & $-$0.238 \\
&D            & 0.002 && 0.009  & $-$0.064  & 0.389  & 0.282  & 0.656  & $-$0.720  & $-$0.541 \\
&D$_p$        & $-$0.258 && $-$0.285  & $-$0.304  & 0.033  & 0.209  & $-$0.226  & $-$0.550  & $-$0.683 \\
&E$_p$        & $-$0.218 && $-$0.152  & $-$0.143  & 0.043  & 0.426  & $-$0.352  & $-$0.702  & $-$0.646 \\
&E            & $-$0.202 && $-$0.063  & $-$0.044  & $-$0.075  & 0.300  & $-$0.346  & $-$0.646  & $-$0.539 \\

%\midrule

%      &       &       &       &       &       &       &       &       &  \bigstrut\\
%\hline
%\multicolumn{10}{c}{Correlation between Rounds 1 and 2} \bigstrut\\
\midrule
\multicolumn{2}{c}{$r$} & 0.969  && 0.952  & 0.927  & 0.899  & 0.960  & 0.951  & 0.646  & 0.936   \bigstrut[t]\\
%\multicolumn{2}{c}{Spearman} & 0.903  && 0.818  & 0.855  & 0.806  & 0.939  & 0.915  & 0.673  & 0.939   \bigstrut[b]\\
\bottomrule
\end{tabular}%


==> tables/tbl-03-corr-free-and-known.tex <==

\begin{tabular}{ccrrrrrrrr}
\toprule
\multicolumn{10}{c}{Free Topic} \bigstrut\\
\midrule
& & \multicolumn{1}{c}{$z$} & \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic} & \rotatebox{60}{Repetitive} \\



%\multicolumn{10}{c}{Known Topic} \bigstrut\\


\midrule
\multirow{8}*{\rotatebox{90}{Known Topic}} 
&$z$            & 0.984 & 0.969  & 0.973  & 0.806  & 0.969  & 0.687  & 0.903  & 0.719 \\
&Interesting            & 0.894 & 0.967  & 0.939  & 0.598  & 0.908  & 0.443  & 0.813  & 0.851 \\
&Fun            & 0.915 & 0.970  & 0.944  & 0.639  & 0.916  & 0.495  & 0.832  & 0.838 \\
&Consistent            & 0.914 & 0.765  & 0.817  & 0.958  & 0.878  & 0.912  & 0.882  & 0.341 \\
&Fluent            & 0.975 & 0.941  & 0.966  & 0.839  & 0.951  & 0.725  & 0.909  & 0.640 \\
&To$_p$ic            & 0.843 & 0.649  & 0.709  & 0.976  & 0.774  & 0.981  & 0.779  & 0.191 \\
&Robotic            & 0.831 & 0.829  & 0.829  & 0.680  & 0.909  & 0.536  & 0.715  & 0.619 \\
&Re$_p$etitive            & 0.721 & 0.876  & 0.825  & 0.317  & 0.713  & 0.151  & 0.650  & 0.950 \\
%      &       &       &       &       &       &       &       &       &  \bigstrut\\
%\hline
%\multicolumn{10}{c}{Correlation between Rounds 1 and 2} \bigstrut\\
%\midrule

\bottomrule
\end{tabular}%


==> tables/tbl-06-corr.tex <==

    \begin{tabular}{crr}
    \toprule

Model                     & Run 1 & Run 2 \bigstrut\\
    \midrule
    A\personafill            & 0.534           & \multicolumn{1}{r}{0.455 } \bigstrut[t]\\
    B\personafill            & 0.419           & \multicolumn{1}{r}{0.344 } \\
    A$_p$                 & 0.318           & \multicolumn{1}{r}{0.423 } \\
    C\personafill            & 0.262           & \multicolumn{1}{r}{0.245} \\
    C$_p$                 & 0.190           & \multicolumn{1}{r}{0.154 } \\
    B$_p$                 & 0.173           & \multicolumn{1}{r}{0.260 } \\
    D\perosnafill                  & $-$0.087  & \multicolumn{1}{r}{0.002 } \\
    D$_p$                       & $-$0.201  & \multicolumn{1}{r}{$-$0.258 } \\
    E$_p$                       & $-$0.217  & \multicolumn{1}{r}{$-$0.218 } \\
    E\personafill                  & $-$0.243  & \multicolumn{1}{r}{$-$0.202 } \bigstrut[b]\\
    \midrule
    $r$                 & \multicolumn{2}{c}{0.969 	} \bigstrut\\
    \bottomrule
    \end{tabular}%







==> tables/tbl-06-corr_bkp.tex <==

    \begin{tabular}{crr}
    \toprule

Model                     & Run 1 & Run 2 \bigstrut\\
    \midrule
    B\autofill                  & 0.4109    & \multicolumn{1}{r}{0.3739} \bigstrut[t]\\
    A$_p$                       & 0.3993    & \multicolumn{1}{r}{0.3223} \\
    A\autofill                  & 0.3826    & \multicolumn{1}{r}{0.5961} \\
    B$_p$                       & 0.2733    & \multicolumn{1}{r}{0.0772} \\
    C\autofill                  & 0.2244    & \multicolumn{1}{r}{0.2445} \\
    C$_p$                       & 0.1981    & \multicolumn{1}{r}{0.2115} \\
    D\autofill                  & 0.0573    & \multicolumn{1}{r}{$-$0.0702} \\
    E$_p$                       & $-$0.2051 & \multicolumn{1}{r}{$-$0.2127} \\
    D$_p$                       & $-$0.2052 & \multicolumn{1}{r}{$-$0.1793} \\
    E\autofill                  & $-$0.2627 & \multicolumn{1}{r}{$-$0.1895} \bigstrut[b]\\
    \midrule
    $r$                 & \multicolumn{2}{c}{0.915} \bigstrut\\
    \bottomrule
    \end{tabular}%





==> tables/tbl-06-old.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Table of z-score}
    \begin{tabular}{ccrc}
    \hline
    \multirow{2}[4]{*}{model} & \multicolumn{3}{c}{z-score} \bigstrut\\
\cline{2-4}          & Free(r1) & \multicolumn{1}{c}{Free(r2)} & Known \bigstrut\\
    \hline
    B\autofill    & 0.4109 & \multicolumn{1}{c}{0.3739} & 0.3241 \bigstrut[t]\\
    A$_p$    & 0.3993 & \multicolumn{1}{c}{0.3223} & 0.4477 \\
    A\autofill  & 0.3826 & \multicolumn{1}{c}{0.5961} & 0.5744 \\
    B$_p$   & 0.2733 & \multicolumn{1}{c}{0.0772} & 0.3004 \\
    C\autofill     & 0.2244 & \multicolumn{1}{c}{0.2445} & 0.3232 \\
    C$_p$    & 0.1981 & \multicolumn{1}{c}{0.2115} & 0.1499 \\
    D\autofill     & 0.0573 & \multicolumn{1}{c}{-0.0702} & -0.1290 \\
    E$_p$    & -0.2051 & \multicolumn{1}{c}{-0.2127} & -0.1649 \\
    D$_p$   & -0.2052 & \multicolumn{1}{c}{-0.1793} & -0.2857 \\
    E\autofill     & -0.2627 & \multicolumn{1}{c}{-0.1895} & -0.2271 \bigstrut[b]\\
    \hline
    Correlation & -     & 0.91523334 & 0.94130859 \bigstrut\\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\small
  \centering
  \caption{Table of automatic metrics from Convai2}
    \begin{tabular}{cccccc}
    Model & Overall & $z$ & F1    & hit$@$1 & ppl$\downarrow$ \bigstrut[b]\\
    \hline
    B$_p$    & 52.41 & 0.2733 & 0.883  & 0.868  & - \bigstrut[t]\\
    A$_p$   & 52.46 & 0.3993 & 0.147  & 0.000  & - \\
    C$_p$ & 48.52 & 0.1981 & 0.598  & 0.551  & - \\
    D$_p$    & 36.59 & -0.2052 & 0.000  & -     & 3.855  \\
    E$_p$    & 35.74 & -0.2051 & 0.153  & -     & 30.510  \bigstrut[b]\\
    \hline
    \multirow{2}[2]{*}{Pearson} & \multicolumn{2}{c}{with overall} & 0.653  & -0.164  & - \bigstrut[t]\\
          & \multicolumn{2}{c}{with z} & 0.537  & -0.733  & - \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tables/tbl-07-metrics.tex <==

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\small
  \centering
  \caption{Table of automatic metrics from Convai2}
    \begin{tabular}{cccccc}
    Model & Overall & $z$ & F1    & hit$@$1 & ppl$\downarrow$ \bigstrut[b]\\
    \hline
    B$_p$    & 52.41 & 0.2733 & 0.883  & 0.868  & - \bigstrut[t]\\
    A$_p$   & 52.46 & 0.3993 & 0.147  & 0.000  & - \\
    C$_p$ & 48.52 & 0.1981 & 0.598  & 0.551  & - \\
    D$_p$    & 36.59 & -0.2052 & 0.000  & -     & 3.855  \\
    E$_p$    & 35.74 & -0.2051 & 0.153  & -     & 30.510  \bigstrut[b]\\
    \hline
    \multirow{2}[2]{*}{Pearson} & \multicolumn{2}{c}{with overall} & 0.653  & -0.164  & - \bigstrut[t]\\
          & \multicolumn{2}{c}{with z} & 0.537  & -0.733  & - \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:metrics}%
\end{table}%

==> tables/tbl-08-corr-with-fed.tex <==
\begin{tabular}{ccccc}
\hline
        & dialogpt-md & dialogpt-lg & bart-base & bart-lg \bigstrut[t]\\
        \hline
    overall & 0.5902  & 0.5300  & 0.1878  & -0.1087  \\
    interesting & 0.0279  & -0.0419  & -0.2154  & -0.2697  \\
    fun   & -0.3390  & 0.1151  & -0.1369  & 0.2437  \\
    consistent & 0.2365  & 0.2270  & 0.0609  & -0.3505  \\
    fluent & -0.1382  & -0.0537  & 0.1957  & 0.2568  \\
    robotic & 0.5282  & 0.4610  & 0.1062  & 0.0165  \\
    repetitive & 0.8415  & 0.7516  & 0.3902  & 0.2978  \\
    topic & 0.0465  & 0.0038  & -0.1296  & -0.4947  \bigstrut[b]\\
\hline
\end{tabular}



==> tables/tbl-11-raw-and-likert.tex <==
%     \begin{tabular}{cccccccccc}
%     \hline
%     \multirow{2}[4]{*}{-} &       & \multicolumn{3}{c}{DA} &       & \multicolumn{4}{c}{Likert (Filtered)} \bigstrut\\
% \cline{3-5}\cline{7-10}          &       & Filtered & Unfiltered & Unqualified &       & 2     & 4     & 5     & 10 \bigstrut\\
% \cline{1-1}\cline{3-5}\cline{7-10}    Overall &       & \underline{0.367}  & 0.214  & 0.015  &       & 0.282  & 0.355  & 0.267  & 0.358  \bigstrut[t]\\
%     Interesting &       & \underline{0.309}  & 0.193  & -0.038  &       & 0.238  & 0.253  & 0.270  & 0.299  \\
%     Fun   &       & \underline{0.323}  & 0.180  & 0.020  &       & 0.246  & 0.289  & 0.299  & 0.314  \\
%     Consistent &       & \underline{0.305}  & 0.170  & 0.003  &       & 0.236  & 0.268  & 0.285  & 0.294  \\
%     Fluent &       & \underline{0.433}  & 0.266  & -0.017  &       & 0.292  & 0.377  & 0.372  & 0.410  \\
%     Robotic &       & 0.102  & 0.056  & -0.010  &       & 0.091  & 0.111  & \underline{0.112}  & 0.103  \\
%     Repetitive &       & \underline{0.223}  & 0.126  & -0.019  &       & 0.210  & 0.225  & 0.214  & 0.217  \\
%     Topic &       & \underline{0.393}  & 0.229  & 0.016  &       & 0.307  & 0.388  & 0.368  & 0.385  \bigstrut[b]\\
%     \hline
%     \end{tabular}


    \begin{tabular}{ccccccccccccccccc}
    \hline
    \multirow{3}[6]{*}{-} &       & \multicolumn{3}{c}{\multirow{2}[4]{*}{DA}} &       & \multicolumn{11}{c}{$n$-point Likert} \bigstrut\\
\cline{7-17}          &       & \multicolumn{3}{c}{}  &       & \multicolumn{2}{c}{2} &       & \multicolumn{2}{c}{4} &       & \multicolumn{2}{c}{5} &       & \multicolumn{2}{c}{10} \bigstrut\\
\cline{3-5}\cline{7-8}\cline{10-11}\cline{13-14}\cline{16-17}          &       & Pass & All   & Fail &       & Pass & Fail &       & Pass & Fail &       & Pass & Fail &       & Pass & Fail \bigstrut\\
\cline{1-1}\cline{3-5}\cline{7-8}\cline{10-11}\cline{13-14}\cline{16-17}    Ovr. &       & \underline{0.367}  & 0.214  & 0.015  &       & 0.282  & 0.049  &       & 0.355  & 0.052  &       & 0.267  & 0.037  &       & 0.358  & 0.047  \bigstrut[t]\\
    Int. &       & \underline{0.309}  & 0.193  & -0.038  &       & 0.238  & 0.048  &       & 0.253  & 0.073  &       & 0.270  & 0.034  &       & 0.299  & 0.027  \\
    Fun.   &       & \underline{0.323}  & 0.180  & 0.020  &       & 0.246  & 0.025  &       & 0.289  & 0.016  &       & 0.299  & 0.021  &       & 0.314  & 0.002  \\
    Con. &       & \underline{0.305}  & 0.170  & 0.003  &       & 0.236  & -0.008  &       & 0.268  & -0.003  &       & 0.285  & 0.011  &       & 0.294  & 0.002  \\
    Flu. &       & \underline{0.433}  & 0.266  & -0.017  &       & 0.292  & 0.037  &       & 0.377  & 0.082  &       & 0.372  & 0.075  &       & 0.410  & 0.057  \\
    Rob. &       & 0.102  & 0.056  & -0.010  &       & 0.091  & 0.013  &       & 0.111  & -0.008  &       & \underline{0.112}  & -0.022  &       & 0.103  & 0.017  \\
    Rep. &       & \underline{0.223}  & 0.126  & -0.019  &       & 0.210  & 0.009  &       & 0.225  & 0.026  &       & 0.214  & 0.003  &       & 0.217  & 0.021  \\
    Top. &       & \underline{0.393}  & 0.229  & 0.016  &       & 0.307  & 0.020  &       & 0.388  & 0.011  &       & 0.368  & 0.026  &       & 0.385  & 0.005  \bigstrut[b]\\
    \hline
    \end{tabular}


% Ovr.
% Int.
% Fun.
% Con.
% Flu.
% Rob.
% Rep.
% Top.

% Overall
% Interesting
% Fun
% Consistent
% Fluent
% Robotic
% Repetitive
% Topic



==> tables/tbl-13-topic-count.tex <==
\begin{tabular}{cc}
Topic & Count \bigstrut[b]\\
\hline
Food  & 72 \bigstrut[t]\\
Movie & 60 \\
Game  & 44 \\
Music & 40 \\
Pet   & 37 \\
Dog   & 31 \\
Car   & 29 \\
Politic & 27 \\
Sport & 24 \\
Animal & 23 \bigstrut[b]\\
\hline
\end{tabular}%



==> tables/tbl-14-kappa.tex <==

\begin{tabular}{ccccccccccccc}
\hline
\multirow{3}[6]{*}{-} &       & \multicolumn{11}{c}{$n$-point Likert rating scale} \bigstrut\\
\cline{3-13}          &       & \multicolumn{2}{c}{2} &       & \multicolumn{2}{c}{4} &       & \multicolumn{2}{c}{5} &       & \multicolumn{2}{c}{10} \bigstrut\\
\cline{3-4}\cline{6-7}\cline{9-10}\cline{12-13}          &       & Pass  & Fail  &       & Pass  & Fail  &       & Pass  & Fail  &       & Pass  & Fail \bigstrut\\
\cline{1-1}\cline{3-4}\cline{6-7}\cline{9-10}\cline{12-13}    Ovr.  &       & 0.165  & -0.017  &       & 0.107  & -0.024  &       & 0.065  & 0.011  &       & 0.040  & 0.010  \bigstrut[t]\\
Int.  &       & 0.146  & 0.029  &       & 0.084  & 0.070  &       & 0.066  & 0.064  &       & 0.049  & 0.035  \\
Fun.  &       & 0.148  & -0.012  &       & 0.089  & -0.015  &       & 0.074  & 0.019  &       & 0.048  & 0.004  \\
Con.  &       & 0.115  & -0.040  &       & 0.078  & 0.037  &       & 0.070  & 0.044  &       & 0.059  & 0.026  \\
Flu.  &       & 0.159  & 0.045  &       & 0.130  & -0.008  &       & 0.108  & 0.051  &       & 0.075  & 0.009  \\
Rob.  &       & 0.010  & -0.028  &       & 0.044  & 0.059  &       & 0.041  & 0.020  &       & 0.034  & -0.016  \\
Rep.  &       & 0.135  & -0.012  &       & 0.077  & 0.010  &       & 0.055  & 0.021  &       & 0.033  & 0.015  \\
Top.  &       & 0.208  & -0.035  &       & 0.141  & 0.016  &       & 0.117  & 0.014  &       & 0.083  & 0.009  \bigstrut[b]\\
\hline
\end{tabular}


==> tables/tbl-15-topic-pairs.tex <==
\begin{tabular}{ccccc}
\hline
\multicolumn{2}{c}{run1} &       & \multicolumn{2}{c}{run2} \bigstrut\\
\cline{1-2}\cline{4-5}    Topic & Pairs &       & Topic & Pairs \bigstrut\\
\cline{1-2}\cline{4-5}    food  & 8     &       & movies & 6 \bigstrut[t]\\
movies & 8     &       & sports & 3 \\
politics & 3     &       & music & 3 \\
dogs  & 3     &       & cats  & 2 \\
music & 2     &       & food  & 1 \\
animals & 2     &       & cooking & 1 \\
kids  & 1     &       & exercise & 1 \\
money & 1     &       & video games & 1 \\
cats  & 1     &       & pets  & 1 \\
sports & 1     &       & reading & 1 \\
school & 1     &       & football & 1 \\
cars  & 1     &       & \multicolumn{2}{c}{-} \\
television & 1     &       & \multicolumn{2}{c}{-} \bigstrut[b]\\
\hline

\end{tabular}

==> tables/tbl-16-sametopic.tex <==

\begin{tabular}{cccc}
\hline
      & N     & n     & percentage \bigstrut\\
\hline
Run 1 & 680   & 33    & 4.85\% \bigstrut[t]\\
Run 2 & 385   & 21    & 5.45\% \bigstrut[b]\\
\hline
\end{tabular}%


==> tables/tbl-18-word-and-char-count.tex <==

%     \begin{tabular}{cc|c|c}
%     \hline
%     \multicolumn{2}{c|}{} & Words per conv & Chars per conv \bigstrut\\
%     \hline
%     \multicolumn{1}{c|}{\multirow{2}[4]{*}{Ours}} & Passed & 68.9  & 275.8  \bigstrut\\
% \cline{2-4}    \multicolumn{1}{c|}{} & Failed & 52.6  & 209.9  \bigstrut\\
%     \hline
%     \multicolumn{2}{c|}{Convai2 Wild} & 42.9  & 166.0  \bigstrut\\
%     \hline
%     \end{tabular}
    




\begin{tabular}{|cc|c|c|}
\hline
\multicolumn{2}{|c|}{} & Words per conv & Chars per conv \bigstrut\\
\hline
\multicolumn{1}{|c|}{\multirow{2}[4]{*}{Ours}} & Passed & 63    & 249  \bigstrut\\
\cline{2-4}    \multicolumn{1}{|c|}{} & Failed & 48    & 188  \bigstrut\\
\hline
\multicolumn{2}{|c|}{Convai2 Wild } & 28    & 105  \bigstrut\\
\hline
\end{tabular}


==> tables/tbl-19-words-uttr.tex <==

%     \begin{tabular}{cc|c|c}
%     \hline
%     \multicolumn{2}{c|}{} & Words per uttr & Chars per uttr \bigstrut\\
%     \hline
%     \multicolumn{1}{c|}{\multirow{2}[4]{*}{Ours}} & Passed & 8.4   & 29.4  \bigstrut\\
% \cline{2-4}    \multicolumn{1}{c|}{} & Failed & 7.2   & 25.0  \bigstrut\\
%     \hline
%     \multicolumn{2}{c|}{Convai2 Wild } & 5.6   & 21.9  \bigstrut\\
%     \hline
%     \end{tabular}



\begin{tabular}{|cc|c|c|}
\hline
\multicolumn{2}{|c|}{} & Words per uttr & Chars per uttr \bigstrut\\
\hline
\multicolumn{1}{|c|}{\multirow{2}[4]{*}{Ours}} & Passed & 8     & 27 \bigstrut\\
\cline{2-4}    \multicolumn{1}{|c|}{} & Failed & 6     & 22 \bigstrut\\
\hline
\multicolumn{2}{|c|}{Convai2 Wild } & 4     & 16 \bigstrut\\
\hline
\end{tabular}


==> tables/tbl-20-autometric-1.tex <==
% \begin{tabular}{lcccccc}
% \hline
% Model & Rouge-L & METEOR & BLEU-4 & BLEU-4 & GLEU  & WER \\
% A     & 12.73  & 6.50  & 1.01  & 15.96  & 4.30  & -0.94  \\
% B     & 11.96  & 6.12  & 0.91  & 14.73  & 4.02  & -0.92  \\
% A\_p  & 13.72  & 7.29  & 1.33  & 16.63  & 4.75  & -0.97  \\
% C     & 11.26  & 5.95  & 0.80  & 13.32  & 3.77  & -1.06  \\
% C\_p  & 11.87  & 6.16  & 0.90  & 14.31  & 3.94  & -0.99  \\
% B\_p  & 13.73  & 7.09  & 1.34  & 16.75  & 4.69  & -0.95  \\
% D     & 15.00  & 6.50  & 1.63  & 16.51  & 4.71  & -0.90  \\
% D\_p  & 16.28  & 7.27  & 2.43  & 18.56  & 5.89  & -0.87  \\
% E\_p  & 14.96  & 6.68  & 2.13  & 18.19  & 5.63  & -0.87  \\
% E     & 14.96  & 6.68  & 2.13  & 18.19  & 5.63  & -0.87 \\
% \hline
% $p$     & -0.799  & -0.321  & -0.883  & -0.707  & -0.816  & -0.641  \\
% s     & -0.705  & -0.328  & -0.766  & -0.705  & -0.681  & -0.669  \\
% k     & -0.494  & -0.225  & -0.584  & -0.494  & -0.494  & -0.539  \\
% \hline
% \end{tabular}%



\begin{tabular}{lccccc}
\hline
Model & Rouge-L & METEOR & BLEU-4 & BLEU-1 & GLEU   \\
A     & 12.73  & 6.50  & 1.01  & 15.96  & 4.30    \\
B     & 11.96  & 6.12  & 0.91  & 14.73  & 4.02   \\
A\_p  & 13.72  & 7.29  & 1.33  & 16.63  & 4.75   \\
C     & 11.26  & 5.95  & 0.80  & 13.32  & 3.77    \\
C\_p  & 11.87  & 6.16  & 0.90  & 14.31  & 3.94    \\
B\_p  & 13.73  & 7.09  & 1.34  & 16.75  & 4.69   \\
D     & 15.00  & 6.50  & 1.63  & 16.51  & 4.71   \\
D\_p  & 16.28  & 7.27  & 2.43  & 18.56  & 5.89   \\
E\_p  & 14.96  & 6.68  & 2.13  & 18.19  & 5.63    \\
E     & 14.96  & 6.68  & 2.13  & 18.19  & 5.63  \\
\hline
$r$     & -0.799  & -0.321  & -0.883  & -0.707  & -0.816    \\
% s     & -0.705  & -0.328  & -0.766  & -0.705  & -0.681    \\
% k     & -0.494  & -0.225  & -0.584  & -0.494  & -0.494   \\
\hline
\end{tabular}%


==> tables/tbl-21-corr-autometric-1.tex <==
\begin{tabular}{lc}
\hline
\multicolumn{1}{c}{Metric} & Correlation \\
\hline
Rouge-L  &  $-$0.799 \\
METEOR  &  $-$0.321 \\
BLEU-4  &  $-$0.883 \\
BLEU-1  &  $-$0.707 \\
GLEU   & $-$0.816 \\
\hline
\end{tabular}%




==> tables/tbl-22-corr-autometric-2.tex <==
% \begin{tabular}{lcccccccc}
% \hline
% % \multicolumn{1}{c}{Pre-tained} & Overall & Interesting & Fun   & Consistent & Fluent & Robotic & Repetitive & Topic \\
% \multicolumn{1}{c}{Pre-tained} & \rotatebox{60}{Overall} & \rotatebox{60}{Interesting} & \rotatebox{60}{Fun} & \rotatebox{60}{Consistent} & \rotatebox{60}{Fluent} & \rotatebox{60}{Topic} & \rotatebox{60}{Robotic } & \rotatebox{60}{Repetitive} \\
% \hline
% DialoGPT-md & 0.590  & 0.028  & -0.339  & 0.236  & -0.138  & 0.046  & 0.841  & 0.528  \\
% DialoGPT-lg & 0.530  & -0.042  & 0.115  & 0.227  & -0.054  & 0.004  & 0.752  & 0.461  \\
% BART-base & 0.188  & -0.215  & -0.137  & 0.061  & 0.196  & -0.130  & 0.390  & 0.106  \\
% BART-lg & -0.109  & -0.270  & 0.244  & -0.350  & 0.257  & -0.495  & 0.298  & 0.016  \\
% RoBERTa-base & -0.577  & -0.705  & 0.023  & -0.162  & 0.349  & -0.048  & -0.924  & -0.439  \\
% RoBERTa-lg & -0.427  & 0.663  & -0.449  & -0.132  & -0.399  & 0.117  & -0.745  & -0.281 \\
% \hline
% \end{tabular}%
\begin{tabular}{lcc}
\hline
      & DialoGPT-md & DialoGPT-lg \\
\hline
Overall & \phantom{$-$}0.590  & \phantom{$-$}0.530   \\
Interesting & \phantom{$-$}0.028  & $-$0.042  \\
Fun   & $-$0.339  & \phantom{$-$}0.115  \\
Consistent & \phantom{$-$}0.236  & \phantom{$-$}0.227  \\
Fluent & $-$0.138  & $-$0.054  \\
Topic & \phantom{$-$}0.046  & \phantom{$-$}0.004  \\
Robotic & \phantom{$-$}0.528  & \phantom{$-$}0.461 \\
Repetitive & \phantom{$-$}0.841  & \phantom{$-$}0.752  \\

\hline
\end{tabular}%


==> tables/tbl-23-corr-autometric-3.tex <==
\begin{tabular}{lcccc}
\hline
 & USR   & USR$_{m}$ & USR$_{c}$ & USR$_{f}$ \\

\hline
Overall     & $-$0.230  & $-$0.419  & \phantom{$-$}0.046  & \phantom{$-$}0.205 \\
Interesting & $-$0.451  & $-$0.235  & $-$0.238  & $-$0.081  \\
Fun   & $-$0.378  & $-$0.319  & $-$0.131  & \phantom{$-$}0.032  \\
Consistent & \phantom{$-$}0.214  & $-$0.620  & \phantom{$-$}0.518  & \phantom{$-$}0.652  \\
Fluent & $-$0.227  & $-$0.374  & \phantom{$-$}0.028  & \phantom{$-$}0.151  \\
Topic & \phantom{$-$}0.222  & $-$0.754  & \phantom{$-$}0.606  & \phantom{$-$}0.746  \\
Robotic & $-$0.070  & $-$0.290  & \phantom{$-$}0.106  & \phantom{$-$}0.191  \\
Repetitive & $-$0.713  & \phantom{$-$}0.182  & $-$0.690  & $-$0.568  \\
\hline
\end{tabular}


